Theory-guided Data Science: A New Paradigm for Scientific Discovery from Data

Data science models, although successful in a number of commercial domains, have had limited applicability in scientific problems involving complex physical phenomena. Theory-guided data science (TGDS) is an emerging paradigm that aims to leverage the wealth of scientific knowledge for improving the effectiveness of data science models in enabling scientific discovery. The overarching vision of TGDS is to introduce scientific consistency as an essential component for learning generalizable models. Further, by producing scientifically interpretable models, TGDS aims to advance our scientific understanding by discovering novel domain insights. Indeed, the paradigm of TGDS has started to gain prominence in a number of scientific disciplines such as turbulence modeling, material discovery, quantum chemistry, bio-medical science, bio-marker discovery, climate science, and hydrology. In this paper, we formally conceptualize the paradigm of TGDS and present a taxonomy of research themes in TGDS. We describe several approaches for integrating domain knowledge in different research themes using illustrative examples from different disciplines. We also highlight some of the promising avenues of novel research for realizing the full potential of theory-guided data science.

==> paper_sections/differences.tex <==
%!TEX root = ../main_file.tex
\section{Differences between traditional and physics-guided data science}\label{sec:diffs}

A variety of domains have advocated for the incorporation of domain knowledge in their methods. These include spatial statistics, GIS, and applied mathematics. What distinguishes theory-guided data science from traditional data science is that the application domain's theory is deep embedded in every step of the knowledge discovery process from data curation to communicating results. In this section, we review some key differences in the knowledge discovery process. We will highlight theory-guided methods in Section \ref{sec:applications}.

\subsection{Data empathy}

Second, with large datasets where one measures anything and
everything, it can be difficult to understand how that data
were collected and for what purpose.
Every dataset has a story, and understanding it can guide the
choice of suitable analyses; some have labeled this data understanding
as data empathy. The reason for understanding
where the data come from is twofold: first, understanding how
the data are generated, their purpose, and generation processes
will guide your investigation. Second, understanding
the inherent biases in the data gives you a chance to correct
them or adjust your results and recommendations.

Data empathy is especially critical in scientific domains where data are large, yet not at the Internet-scale of billions or trillions of observations. In such a case, the data's size is not enough to smooth over any biases in data collection or processing.

For example, one of the most widely used datasets in machine learning is the mushroom dataset from the UCI repository. This dataset is commonly used to demonstrate a basic classification problem of predicting whether a mushroom is
edible (i.e., poisonous or not) based on some physical features. The dataset comes with two labels, ``poisonous'' and ``not poisonous''; however, reading the data's description, we find that ``Each species is identified as definitely edible, definitely poisonous, or of unknown edibility and not recommended. This latter class was combined with the poisonous one'' (see \url{https://archive.ics.uci.edu/ml/datasets/Mushroom}).
Thus, the data originally had three classes that were collapsed into two.
In this particular case, the best models are, therefore, guaranteed to yield false positives, where a mushroom is labeled as poisonous while it is not. But consider the disastrous impact if these uncertain mushrooms were merged with the nonpoisonous class instead.

\subsection{Data representation}
At a high level, data science and more specifically data mining and machine learning methods are primarily designed to work with attribute-value data representation \cite{Tan2005,langley2011}. However, numerous climate phenomena are dynamic and spatio-temporal and hence cannot be represented in attribute-value form. This makes predictions difficult as we often abstract phenomena into an attribute-value form that may cause a loss of critical information. Other data representations are becoming increasingly popular such as manifold and topological representations. However, to take advantage of such representations we must first constrain them by the physics that govern Earth Science observations. This is because in the case of predictive models of systems governed by physical laws, understanding the operating regime of the physical variables is necessary to make meaningful predictionsFor example, a physics-based constraint connecting a few variables would imply that the variables of interest can only span a manifold embedded in the ambient space, so using methods which assume the span to be the full Euclidean space is misdirected. Thus the observations (predictors) may live in a high-dimensional ambient system, but the physical laws governing the system constraints them to live in a suitable subset, possibly a manifold embedded in the ambient space. Thus, for a given physical system, one needs to consider, possibly learn, a suitable representation for the constrained space in which the physical variables live.

% \subsection{Methods}
% How does Physics-aware data science differ from traditional data-science and feature selection? These may use Physics theories as constraints on data science methods. It is a dual of ``data constraining Physics models" in terms of initial conditions and boundary conditions. Physics-constraints on data science methods gives arise to newer semantics for traditional pattern families. For example, Physics-aware anomalies may be identify as data-elements (e.g., locations, time) violating laws of Physics to detect shears, spikes, cracks, tears, wrinkles, contact-problems \cite{bradley2004}

% Physics-aware clustering may identify hot-spots (and time-intervals) of physics-aware anomalies. This may be used to identify turbulent flows \cite{tmc2014} and other spatio-temporal regions where current laws of Physics do not adequately model the local phenomena. Physics-aware (sequential-) association rule miners may look for frequent (or high-confidence) co-occurrence of physics-aware anomalies/clusters and geophysical features such as surface discontinuities and roughness.

% Physics-aware classification and prediction methods (e.g., decision trees) may explore ways to forecast violations of current laws of Physics based a combination of factors using simple big-data approaches (e.g., nearest neighbor in parameter space) or ensemble models.

% Algorithms for mining clusters, association and predictive models may also be constrained to focus on climate patterns obeying laws of Physics. Mining of climate features such as polar vortex, atmospheric rivers and
% ocean eddies may need new generation of physics-constrained clustering techniques to be effective \cite{faghmous2012cidu}.

% Richer set of Physics concepts may also be used for the feature selection to benefit both Physics-aware data science and traditional data science \cite{ganguly2014}.

\subsection{Flexibility vs. Interpretability}
An important consideration for a data driven approach in the context of climate informatics is the dichotomy between accuracy and interpretability. Unlike applications where accuracy is the primary goal, in the context of climate, achieving somewhat accurate projections without a mechanistic understanding of the underlying climatic and hydrological processes is problematic, and can- not serve as a basis for sub- sequent developments. The challenge in developing such a mechanistic understanding is that the climate system has a wide range of nonlinear and conditional dependencies. Understanding such dependencies, based on data driven methods, is a necessary step towards characterizing the structural constraints under which the climate system operates, which in turn will guide the development of interpretable data driven models for climate data analysis.

\subsection{Results interpretation}
The final step in any data science investigation is interpreting the results. Generally speaking, each investigator has processes and a lens by which she interprets results. In the case of climate however, the results interpretation lens must be grounded in the basic physical theories that govern the Earth System. For example, if a sparse regression model that takes into account thousands of predictors and then only selects a handful, yet the predictors that cannot possibly influence the phenomenon of interest (for a physics standpoint), then one must reconsider such results. So if one of the predictors selected (out of 1,000s) to predict  hurricane occurrence in the North Atlantic is rainfall in the South Pole with a 2-week lead time, we must reconsider these results as there is no sound physical theory that could explain such influence.

\subsection{Results communication}
The final step in a knowledge discovery paradigm is communicating results. Traditionally, such results can be newly discovered knowledge or a method's performance (e.g. classification error). The main difference between traditional and theory-guided data science is reporting risk and uncertainty. In mainstream data science applications such as recommender systems a poor recommendation might frustrate a user, however miscalculating a rocket's trajectory by a few centimeters can be disastrous.




==> paper_sections/information.tex <==
\section{Different types of domain knowledge}\label{sec:info}

Domain knowledge available in different domains has several characteristics. These characteristics include the granularity of information, type of information, nature of representation,  degree of completeness, uncertainty in the knowledge, and degree of validation. Due to these diverse characteristics, all domain knowledge is not necessarily the same and so incorporating existing domain knowledge to guide the data science process requires the data scientist to be cognizant of these characteristics and the challenges that these characteristics bring forth. %In this section we describe these characteristics and provide examples of such domain knowledge and relevant applications for theory guided data science. 

While domain knowledge in some domains is available at a finer level of detail of the underlying process in the form of first principles, it is available as abstract concepts in other domains. An example of first principles is a quasi-static electromagnetism that explains how the cardiac bioelectric signal is distributed in the human torso [1]. These principles are crucial for reconstructing the flow of cardiac bioelectric signals in the heart volume based on the ECG signal that is measured outside the torso to study clinical problems such as cardiac arrhythmia and heart failure [2]. These principles are represented as partial differential equations. Other examples for first principles are the Newton's laws of motion in physics that can be used to capture of motion of an aircraft. An example of a high-level principle is that changes in the genetic information are known to affect gene expression, protein structure, function, and metabolite levels. This example from the domain of genomics is useful in the discovery of underlying factors for complex diseases. These high level principles are typically represented in flow-charts or described in sentences.

There also exists domain knowledge that falls between the two extremes of first principles and high level principles. Domain knowledge that captures the different process and the relationships between processes can be of multiple types and can have its own suitable representations. One type of information is associations or groups that capture entities that share similar properties or that belong to the same processes. Examples include, proteins with similar function in biology, brain locations with similar functions, streets with similar capacity in transportation, and materials with similar chemical composition in material science. Such information is typically represented as sets.

Another type of information is a relationship between different entities or processes. Examples include, relationship between distant brain regions in neuroscience and long-distance relationships (also referred to as teleconnections) in climate science. In some cases the relationship can also be directional. Examples are, one gene enables the expression of another gene and the direction of traffic on a street. Another example of a directional relationship is that of a membership of a biological function in a more general class of functions (as specified in Gene Ontology). Relationships can also have signs, i.e, positive or negative. An example is the transcriptional relationship of a gene where a gene can enhance the expression of another gene or suppress it. Network representation is ideally suited for this type of domain knowledge that captures relationships.

Yet another type of information are rules that determine how a process is manifest. For example, KEGG pathways that characterize how multiple chemical compounds combine to result in one or more chemical compounds are represented as rules. 



%\textbf{Granularity of information:} While domain knowledge in some domains is available at a finer level of detail of the underlying process in the form of first principles, it is available as abstract concepts in other domains. An example of first principles is a quasi-static electromagnetism that explains how the cardiac bioelectric signal is distributed in the human torso [1]. These principles are crucial for reconstructing the flow of cardiac bioelectric signals in the heart volume based on the ECG signal that is measured outside the torso to study clinical problems such as cardiac arrhythmia and heart failure [2]. Other examples for first principles are the Newton's laws of motion in physics that can be used to capture of motion of an aircraft. An example of a high-level principle is that changes in the genetic information are known to affect gene expression, protein structure, function, and metabolite levels. This example from the domain of genomics is useful in the discovery of underlying factors for complex diseases. 

%\textbf{Type of information:} Domain knowledge that captures the different process and the relationships between processes can be of different types. One type of information is associations or groups that capture entities that share similar properties or that belong to the same processes. Examples include, proteins with similar function in biology, brain locations with similar functions, streets with similar capacity in transportation, and materials with similar chemical composition in material science. 

%Another type of information is a relationship between different entities or processes. Examples include, relationship between distant brain regions in neuroscience and long-distance relationships (also referred to as teleconnections) in climate science. In some cases the relationship can also be directional. Examples are, one gene enables the expression of another gene and the direction of traffic on a street. Another example of a directional relationship is that of a membership of a biological function in a more general class of functions (as specified in Gene Ontology). Relationships can also have signs, i.e, positive or negative. An example is the transcriptional relationship of a gene where a gene can enhance the expression of another gene or suppress it.

%Yet another type of information are rules that determine how a process is manifest. For example, KEGG pathways that characterize how multiple chemical compounds combine to result in one or more chemical compounds are represented as rules.

%\textbf{Nature of representation:} First principles such as quasi-static electromagnetism and Maxwell equations in electrodynamics are represented as mathematical equations and partial differential equations. Sets are a natural representation for domain knowledge that is in the form of associations or groups. Interactions between different entities and processes are typically represented in the form of networks. Rules are another representation for capturing metabolic pathways. Some high-level concepts are also represented using flow charts. For example, the dependence of gene expression, protein structure, and function on genetic information is typically represented as a flow chart.


==> paper_sections/issues.tex <==
\section{Issues in theory-guided data science}\label{sec:issues}

\textbf{Dealing with Incomplete domain knowledge}
Domain information can be complete or incomplete is several domains. In man made systems such as transportation networks and communication networks, the information is generally complete. Where in natural systems such as biology, the information of protein networks, regulatory networks, and gene function is typically incomplete. In such cases, incorporation of domain knowledge as part of the data-driven discovery process is not straight forward. Suitable approaches that can handle incompleteness needs to be investigated.

\textbf{Uncertainty in domain knowledge}
Information that is available in some domains is more reliable than in other domains. For example, the chemical properties of materials in material sciences are generally reliable. Wheres in genomics, the reliability of an interaction between two proteins varies with the technology that is used to capture the interaction. Often, a reliability score is also provided along with each protein interaction. In the case of genetic interactions, the existence of a relationship is typically determined based on the strength of the reliability score. TGDM approaches have to be handle these cases where domain knowledge is uncertain and uncertainty is not quantified, as well as cases where uncertainity is quantified.

\textbf{Data representation}
At a high level, data science and more specifically data mining and machine learning methods are primarily designed to work with attribute-value data representation \cite{Tan2005,langley2011}. However, numerous climate phenomena are dynamic and spatio-temporal and hence cannot be represented in attribute-value form. This makes predictions difficult as we often abstract phenomena into an attribute-value form that may cause a loss of critical information. Other data representations are becoming increasingly popular such as manifold and topological representations. However, to take advantage of such representations we must first constrain them by the physics that govern Earth Science observations. This is because in the case of predictive models of systems governed by physical laws, understanding the operating regime of the physical variables is necessary to make meaningful predictions. For example, a physics-based constraint connecting a few variables would imply that the variables of interest can only span a manifold embedded in the ambient space, so using methods which assume the span to be the full Euclidean space is misdirected. Thus the observations (predictors) may live in a high-dimensional ambient system, but the physical laws governing the system constraints them to live in a suitable subset, possibly a manifold embedded in the ambient space. Thus, for a given physical system, one needs to consider, possibly learn, a suitable representation for the constrained space in which the physical variables live.


\textbf{Results interpretation}
The final step in any data science investigation is interpreting the results. Generally speaking, each investigator has processes and a lens by which she interprets results. In the case of climate however, the results interpretation lens must be grounded in the basic physical theories that govern the Earth System. For example, if a sparse regression model that takes into account thousands of predictors and then only selects a handful, yet the predictors that cannot possibly influence the phenomenon of interest (for a physics standpoint), then one must reconsider such results. So if one of the predictors selected (out of 1,000s) to predict  hurricane occurrence in the North Atlantic is rainfall in the South Pole with a 2-week lead time, we must reconsider these results as there is no sound physical theory that could explain such influence.


%\textbf{Completeness:} Depending on the gaps in the available domain knowledge, it is either complete or incomplete. Typically first principles and knowledge pertaining to man-made systems are deemed complete, whereas most other forms of high-level principles are incomplete. On the other hand, high-level principles and concepts that are discovered from natural systems are typically incomplete. For example, in biological studies, a protein interaction network captures interactions between proteins. In this network, only some of the interactions are known. On the other hand, in transportation studies, a road network captures the network of roads and freeways in any given area. Unlike the protein networks, here all edges (roads) are known.

%\textbf{Certainty:} Certainty in the domain knowledge can vary irrespective of the granularity and type of information. For example, some climatic models constructed based on first principles may capture the climate system more accurately than others. Similarly, certainty can be high for some domain knowledge that are typically high-level concepts. [Need to add an example here.]

==> paper_sections/new_data_science.tex <==
%!TEX root = ../main_file.tex
\section{A new data science paradigm}
\subsection*{Defining the discipline of data science}
We define data science as: ``the extraction of knowledge about models, processes, and phenomena in nature (real-world) by combining first principles with observed data and data analysis methods''. This is different than the \emph{de facto} machine-learning-centric data science definition from section \ref{sec:background}. First, the emphasis is on novel understanding and theory not on increased accuracy at a task. Additional knowledge and understanding might yield better predictive models but developing more accurate models is not an end in itself. Second, this definition of data science is not data-driven only but a combination of domain theory, data, and new hypotheses. Finally, this definition does not tie any discoveries to the size of the data. In fact, we believe in a new era of data science where we need less data and more science.

\subsection{The data science knowledge discovery paradigm}


==> paper_sections/potential_contributions.tex <==
%!TEX root = ../main_file.tex
\section{Data-Driven Global Change Challenges}
\label{sec:applications}
In this section, we continue highlighting some of the differences between traditional and theory-guided data science.

%Climate models have reached significant limitations both computational and conceptual that open the door for data science to make long-lasting contributions. Below are a few possibilities. These are areas that can help us further our understanding of the planet.

%[Note: Prof. Kumar -- Ideally I would like each of these bullet-points to follow the same format for consistency and to stay focused. For example, maybe start with the societal merit, then challenges, then methods. I don't have a format yet but hope to come up with one with your help].



\subsection{Data integration}
Various phenomena of the Earth system are observed using instruments, ground inspections, or Earth-orbiting satellites. One challenge that data-driven global change faces is the record length of any one observation source. Data integration is a common data mining application (citations?) however it differs from a physically-consistent data integration in a few ways. First, the final homogenized product must obey the first principles governing the data. Second, the data's spatio-temporal variability must also be accurately captured in the final product. Finally, prior knowledge about some of the source data and their instruments might be necessary to weight the contribution of each dataset accordingly.

 There are three ways such data integration might manifest in practice: first, in the case of similar instruments as part of different missions. For instance, satellite missions have on average a five-year lifespan, after which new instruments are used with different biases, measurement errors, or even measurement capabilities. In this case, one is interested in integrating the observations from different missions as a single homogeneous record \cite{Srivastava2005}. Second, certain phenomena can be observed from multiple perspectives each with their own uncertainties. For example, ocean surface temperatures can be collected from ships, floats, satellites,  model-observation hybrid products (known as reanalysis), and proxy data such as coral reefs. In this case, we are interested in take multiple noisy, incomplete, and uncertain measurements of the same variable and construct a homogenized spatio-temporal product. This problem will continue to grow as data collection devices continue to be come affordable and ubiquitous as seen with the rapid growth of wearable technology and three-dimensionally printed satellites (\emph{e.g.} CubeSat). Some novel approaches to this problem include \emph{data ensembles} where multiple views of the same data allow to account for joint uncertainties \cite{Sanso2014}. A third and final type of data integration is that of unobservable phenomena. While an eclectic group of phenomena are observed on a global scale, and equal number of other phenomena are not. For example, global forest fires is a critical component to understanding land cover change and its effects on the planet. Yet there is no directly observable ``fires'' product. Instead, we must rely on proxy variables that are known to respond to forest fires. These include: air temperature, land surface temperature, vegetation density, air smoke, etc. What makes this integration challenging is that fires impact each proxy at different spatio-temporal scales hence even detecting the target-proxy relationship can be a challenge. The goal is to combine each proxy signature to get a presence/absence score for a phenomena based on its expected signature in various datasets where some information may be redundant across datasets (i.e. not independent).

\subsection{Data reconstruction -- Arindam could you please expand on this section or improve it as you see fit? I remember you had some work in Paleo}
There is a major need to extend the record for numerous global change datasets since many datasets have only been collected in the past fifty years when global change has been well underway. Since climate observations are available only as far as the mid-19th century, one promising avenue is the use of proxy information such as tree rings and ice cores to infer past climate using the present-day observed relationship between climate variables and said proxies. Of particular interest is re-constructing climates from the Common Era (CE; \~ last two millennia) to study the relationships between climate and societies. Given the large number of proxies, paleoclimate reconstruction can be thought of as a data assimilation problem, given a set of incomplete and uncertain data how can we combine them into a homogenized dataset? Another potential data science contribution could be in the form of matrix completion where given a set of sparse observations one tries to complete the missing data. However, unlike traditional matrix completion problems for image inpainting or recommender systems (citations), here one needs to account for the spatial and temporal variability in the field of interest to produce not only physically consistent output but also to capture some of the long-scale temporal variability that is of interest to many researchers (i.e. the exact values at any one time-step might not matter as much as the collective long-term behavior of the data).

\subsection{Feature selection -- Nagiza could you please contribute some of your work on network-based feature selection?}
[From Shashi write-up] Richer set of Physics concepts may also be used for the feature selection to benefit both Physics-aware data science and traditional data science \cite{ganguly2014}.

\subsection{Unsupervised pattern mining}
In order to be able to adequately manage our resources under global change, we must have systems to autonomously monitor resources on a global scale. While there are numerous global satellite products, we are sometimes interested in phenomena that are not explicitly monitored, yet must be cataloged for either scientific or policy reasons. The biggest challenge when mining patterns on a global scale is natural variability, which causes patterns for the event of interest to be significantly different across space and time. For example, mesoscale ocean eddies are ubiquitous rotating features in the ocean that dominate its kinetic energy and play a role in mitigating climate change. Thus there is a need to monitor such phenomena to understand their global properties but also study their interactions with other components of the Earth System. To address this need, \cite{faghmous2013icdm} proposed a global parameter-free spatio-temporal patten mining algorithm that isolates eddies as closed-contour anomalies in sea level anomalies data. Unlike traditional patterns mining algorithms, the pattern search space can rapidly explode as spatio-temporal patterns manifest in exponentially many spatio-temporal spans. For instance in climate science, phenomena span anywhere between $10^{-6}$m (microns) and $10^{8}$m (the order of Earth's size) in space and $10^{-3}$s to $10^11$s in time. Hence it is not feasible to search for patterns that can be embedded in any combination of the fourteen orders of magnitude in both space and time. Instead we must rely on first principles to not only significantly reduce the search space but also prune out features that might seem statistically significant yet physically-inconsistent. A physically-consistent pattern mining method resulted in the production of the largest open global ocean eddies dataset \cite{dryad_gp40h}, that can be downloaded and used for additional studies.

\subsection{Unsupervised change detection -- Anuj}
Change detection focuses on discovering significant deviations from normative data values. Similar to pattern mining, various spatio-temporal changes are associated with phenomena that we might be interested in yet cannot be directly monitored. For instance, global forest cover have tremendous societal, ecological, and environmental impacts. Yet, there are no reliable and quantifiable observations of changes in forest cover as a result of urbanization, forest fires, or deforestation. Monitoring such changes can be useful for managing forest resources and mitigating ecosystem disturbances as well as for conducting climate change and carbon cycle studies. However, the availability of vast and ever-growing volumes of remote sensing data provides an opportunity for monitoring the health of forests in a spatially explicit and temporally frequent manner. This includes the use of optical remote sensing signals that capture information about the visible, infrared, and thermal parts of the electromagnetic spectrum that can be used for monitoring changes in the forest cover. As an example, vegetation indices that are  computed as non-linear combinations of the opitcal remote sensing signals, such as the Enhanced Vegetation Index (EVI), can be used as a proxy for the amount of ``greenness" at a particular location at a given time. Ecosystem diturbances can then be observed as spatio-temporal changes in the vegetation index datasets, where every type of ecosystem disturbance has its own characteristic signature of change.

The detection and characterization of ecosystem disturbances can them be framed as pattern mining problems where the pattern of interest is the characteristic signature of change of a particular disturbance event. As an example, damage due to insect infestation leads to a slow degradation of the forests, observed as a gradual decrease in the vegetation index. On the other hand, forest fires result in an instantaneous and sharp drop in the vegetation index followed by an interval of gradual recovery of vegetation. However, a major challenge in detecting and characterizing ecosystem disturbances is the presence of a natural variability in the remote sensing observations that is different for different regions on the Earth and different seasonal cycles in the year. An unsupervised algorithm for spatio-temporal change detection thus has to be cognizant of the spatial heterogeneity and temporal variability in the remote sensing datasets, by tuning its model parameters according to the context of the observations at a given location and at a given time-step. Change detection algorithms further have to be resilient to the high degree of noise and outliers present in remote sensing data, along with utilizing information about the spatio-temporal characteristics of ecosystem disturbances, such as spatial coherence, and temporal consistence and persistence. In our previous work, we have a developed a suite of algorithms for addressing the aforementioned challenges and detecting a variety of ecosystem disturbances, such as changes in cropping patterns \cite{garg2011model}, insect damage \cite{chamber2011novel}, deforestation \cite{mithal2011incorporating}, and forest fires \cite{chen2012new}. A comprehensive review on global land cover monitoring using data mining approahces is presented in \cite{mithal2011monitoring}.

\subsection{Data abstraction}
Given their large size and high dimensionality an exhaustive data-driven analysis using all the quantities involved in global change is infeasible. Hence, there is an opportunity to abstract these data in a compact manner without losing their most meaningful features. Traditional techniques such as PCA are well established. Within the spatio-temporal domain empirical orthogonal functions (EOF) have been a popular method for studying the largest sources of variability in space and time. However, these methods have their advantages and limitations and there is ample room for creativity.
For example, it has been proposed to abstract climate data into climate networks where each node is a geographic location and each edge represents the correlation between two nodes \cite{steinhaeuser2011complex}. Using this compact representation, it is now possible to investigate how various climate variables interact \cite{steinhaeuser2012multivariate} as well as compare between various global climate models \cite{steinhaeuser2014climate}. Furthermore, once the data have been abstracted into netwrok form one can apply tradition data mining techniques such as community detection, prediction, or classification \cite{faghmous2013stdm}. Efficient and accurate data abstraction is particularly useful in summarizing climate model output data that may product a simulation of the global climate system at the minutes or hours time-scales. However, given the extreme I/O costs of simulating centuries of the climate system, models generally save to disk at monthly time-scales. Hence rare events such as extreme rainfall are washed out when averaged over an entire month.


\subsection{Spatio-temporal smoothing -- Ansu and Auroop could you please expand on this section?}
Global change data are often incomplete. The reasons for incomplete data sets in global change can be due to to obstructed data or failing instruments, which are not uncommon in other domains. However, other reasons for missing can could be geo-political conflicts, or the potential value of the data themselves such that a {\it missing at random} assumption may not be appropriate. For example, the truncation or absence of data on the height of a river may be due to a potential flood or drought condition, which may itself be the object of study. Not accounting for truncation, censoring, or missing-not-at-random properties of the data may lead to biased results, and greatly affect precision and accuracy statements. Since future measurements may be made without awareness of potential bias and inaccuracy in current data, such inaccuracies may not be identified till considerable harm has been done. Hence, the objective of spatio-temporal smoothing is to ``fill'' missing data in space, time, or both in physically consistent manner.

The most common approach for spatio-temporal smoothing involves assumptions of Gaussian random field for the feature $Y (s, t)$, and much attention is given to specifying parameter structures of such random fields. Since a fully accurate specification is often impossible and because Bayesian statistical methods are commonly in use, hierarchical model specification is also common in spatio-temporal modeling \cite{katzfuss2011spatio, katzfuss2012bayesian}. Generally, hierarchical Bayesian modeling is compatible with domain-guided restrictions on the model. These are usually incorporated as part of the {\it prior specification}. Most modern Bayesian models require extensive computation for the extraction of a sample from the posterior distribution, and domain-guided knowledge and constraints may result in loss of speed and efficiency of computational algorithms. Another alternative is to use penalization methods appropriately (e.g. \cite{lee2011p}). Similar approaches have been used for longitudinal and mortality data by \cite{biatat2011hierarchical}, and for flexible regression in river systems by \cite{odonnell2014flexible}. A large body of literature assume a {\it separable} form, where spatio-temporal dependence is factorizable into two parts, one a function space only and another a function of time \cite{macnab2001autoregressive, kneib2006structured}. However, non-separable models may be better representative of the properties of the data and physical system under study.
A common data science technique to in-data filling is matrix completion \cite{candes2009exact}. However, such a technique would not work in the case of spatio-temporal data since observations are dependent in space and time. Instead, one promising avenue of research is the use of auxiliary variables to infer missing data. For example, if one is trying to fill missing carbon observations in a continuous spatio-temporal field, one could learn from the spatio-temporal patterns between carbon and other auxiliary variables to infer a physically consistent fill value. In a similar vein, one may use the physical process at hand to fill in various parts of the data. For instance, if one is trying to estimate water quality levels in a river where we only have sparse samples. One could use the spatio-temporal flow or velocity of change to infer how the observations from the samples would proagate downstream. Finally, there is the notion of non-seprabale models (i found this paper \url{http://link.springer.com/article/10.1023%2FA%3A1014075310344})

\subsection{Multi-(climate)-model ensembles -- Auroop I know you have been particularly interested in this topic. Could take care of this section?}
The U.N. IPCC relies on a two-dozen global climate models -- physics-based numerical simulations -- to asses global climate change and its risks. Each model has its own paramterization and limitations, and as a result resolves certain processes better than others. [I am not familair with the multi-model problem, may Auroop can give us write-up]

\subsection{Spatio-temporal predictive models -- Anuj + Arindam}
Spatio-temporal predictive models can be used for estimating a variety of ecosystem variables at a given location and time using spatio-temporal remote sensing variables as input features. For example, the target variable of interest can be the amount of forest cover at a given location in a year, which is the amount of pixel area covered by forests (ranging from 0 to 1), which can be estimated using its corresponding land surface temperature observations. However, there exists a rich variety in the relationships between remote sensing variables and the target variable of interest, due to differences in geographies, topographies, and climatological conditions in different regions of the Earth. This results in the presence of a heterogeneity in the data, as different sub-populations of data instances show varying characteristics of the mapping function from the covariates to the target variables. As an example, locations that belong to different vegetation types or land covers show varying characteristics in their relationship between land surface temperature observations and the amount of forest cover, resulting in heterogeneity in the data due to the presence of multiple vegetation types. In such scenarios, one can potentially utilize information about the context of a data instance, such as its location, time of observation, or temporal behavior in the past, for partitioning the heterogeneous dataset into homogeneous groups, which share a common relationship between the covariates and the target variable. In our previous work \cite{karpatne2012importance}, we have explored the use of vegetation index time series at a location, that capture information about the vegetation type at that location, as the relevant contextual information for partitioning the data into homogeneous groups and learning a different model for every such group. However, in a number of real-world scenarios, obtaining labeled data is time-consuming and expensive. In the presence of limited training data, learning a model at every group independently of the other models learned at other groups leads to an increase in the overall model complexity, making the learning prone to over-fitting, which results in poor generalization performance. In order to incorporate the data heterogeneity in the predictve modeling framework along with constraining the model complexity, we have explored regularization techniques that are able to utilize the structure among the groups of data instances, discovered using hierarchical  clustering approaches \cite{datapredictive}. This has applications in a number of real-world predictive modeling scenarios that involves heterogeneous spatio-temporal datasets with limited training data.

As another example of predictive modeling approaches for monitoring ecosystem resources, let's consider the problem of monitoring water bodies using optical remote sensing datasets. This can be formulated as a classification problem where the remote sensing signals are the discriminatory attributes that can help estimate the class label of every pixel at every time-step as either water or land. However, the performance of state-of-the-art classification techniques is impacted the presence of high degree of noise and outliers in remote sensing datasets leading to inconsistencies in performance. However, an understanding of the physical properties of water bodies provides an opportunity for developing theory-guided data science approaches that produce physically consistent results, which can potentially overcome the impact of noise and outliers. As an example, the waterbeds of naturally occurring water bodies are commonly concave in shape, which implies that locations at a lower elevation in the water body will filled with water before locations at a higher elevation are filled with water. This physical understanding of water bodies enforces an ordering among locations and time-steps which can be incorporated in a supervised learning framework as additional constraints. However, obtaining information about elevation is expensive, and existing global scale evelation datasets are only available at coarser resolutions, making them unfit for use in an operational setting. It is thus important to simultaneously estimate the elevation information of locations using temporal context and utilize it for estimating the class label at a given location at a given time-step using theory-guided constraints.


\emph{Lifted from Arindam's write up for IEEE Computer}
Take the example of predicting temperature over Brazil using numerous climate variables. The challenge in predicting climate phenomena is that the Earth is a dynamic system with interconnected components. Thus, a phenomenon such as temperature may have local, long-range, and time-lagged influences. Assume that one is interested in predicting the temperature at monthly time-scales. Hence, for a period of 30 years we would have $n=30 \times 12$ observations. Now consider that a host of locations and time-scales may impact temperatures. Figure \ref{fig:data_example} shows a common data representation used for predictive models. Climate data are represented in a gridded form where each grid point is a location. One of the most commonly used climate datasets, NCEP from the National Center for Atmospheric Research, has a 10,000 grid-point resolution. Each grid-point has twelve monthly observations for each of the thirty years and there are numerous variables that might impact temperature in Brazil such as wind, rainfall, etc. Let number of such variables be $v$. Thus the number of predictors is $ d= 10,000 \times 30  \times 12 \times v$ which is several orders of magnitude larger than $n$ ($d>>n$).

In practice, only a small number of these $d$ predictors may be relevant, and methods such as regularized regression would select a handful of predictors out of a large set. Yet, these techniques fail to account for the dependence between variables and can potentially select predictors that have a high statistical relationship but little physical meaning \cite{caldwell2014statistical}. Motivated by such observations, a group sparse regularizer was presented in \cite{chatterjeeSBCG12}. It first selects the most relevant ocean regions and then selects the climate variables in each relevant ocean region (see Figure \ref{fig:predict_example}). Such hierarchical feature selection incorporating domain knowledge gives more meaningful predictors compared to a simple regression or even an unstructured sparse regression such as LASSO. Such a shift from primarily focusing on accuracy metrics irrespective of what predictors are used to more meaningful domain inspired structures for predictive modeling is a key step in theory-guided data science.

While the preliminary results show promise, the models need to be made considerably more physics informed to yield significant advances in our understanding of the Earth system. For example, instead of directly using climate variables as predictors, the models need to start considering climate processes which determine the spatio-temporal behavior of climate variables. The challenge here is that climate processes are complex phenomena, often involving interactions between atmosphere, ocean, and land dynamics, modulated by climate oscillators, long-range dependencies, and nonlinearity. The move from purely statistical approaches to theory-guided data science needs to start taking such physical processes into account for meaningful data analysis.

\subsection{Large-scale relationship mining}
Using these global-scale datasets there is tremendous interest in capturing the co-occurrences, relationships, and interactions between large-scale variables in the Earth System. For example, there is significant interest in understanding how do large-scale changes in ocean temperatures on a global-scale affect fires in the Amazon. The biggest challenge large-scale relationship mining tasks is that if taken individually each location is likely to be correlated with another location by random change given the large number of tests (in the order of 100 million). In this setting, \cite{kawale2013graph} identified pressure dipoles in global climate data. Pressure dipoles are important long distance climate phenomena (teleconnections) characterized by pressure anomalies of the opposite polarity appearing at two different locations at the same time. Such dipoles have been proven important for understanding and explaining the variability in climate in many regions of the world, e.g. the El Ni\~{n}o Southern Oscillation (ENSO) climate phenomenon, which is described by opposite pressure anomalies between the west and east Pacific and is known to be responsible for precipitation and temperature anomalies worldwide. This work was novel because it automatically identified the highly correlated regions while being robust against spurious correlations \cite{kawale2012testing}
[This work was  also novel because such teleconnections although are known their impacts are diverse depending on how these teleconnections are defined. `I am making this up but I assume it's true]





